Fast and Post-Quantum Authentication for Real-time Next Generation Networks with Bloom Filter

Large-scale next-generation networked systems like smart grids and vehicular networks facilitate extensive automation and autonomy through real-time communication of sensitive messages. Digital signatures are vital for such applications since they offer scalable broadcast authentication with non-repudiation. Yet, even conventional secure signatures (e.g., ECDSA, RSA) introduce significant cryptographic delays that can disrupt the safety of such delay-aware systems. With the rise of quantum computers breaking conventional intractability problems, these traditional cryptosystems must be replaced with post-quantum (PQ) secure ones. However, PQ-secure signatures are significantly costlier than their conventional counterparts, vastly exacerbating delay hurdles for real-time applications. We propose a new signature called Time Valid Probabilistic Data Structure HORS (TVPD-HORS) that achieves significantly lower end-to-end delay with a tunable PQ-security for real-time applications. We harness special probabilistic data structures as an efficient one-way function at the heart of our novelty, thereby vastly fastening HORS as a primitive for NIST PQ cryptography standards. TVPD-HORS permits tunable and fast processing for varying input sizes via One-hash Bloom Filter, excelling in time valid cases, wherein authentication with shorter security parameters is used for short-lived yet safety-critical messages. We show that TVPD-HORS verification is 2.7x and 5x faster than HORS in high-security and time valid settings, respectively. TVPD-HORS key generation is also faster, with a similar signing speed to HORS. Moreover, TVPD-HORS can increase the speed of HORS variants over a magnitude of time. These features make TVPD-HORS an ideal primitive to raise high-speed time valid versions of PQ-safe standards like XMSS and SPHINCS+, paving the way for real-time authentication of next-generation networks.

==> Bodies/models.tex <==
\section{Models}

\noindent \textbf{System Model:} Our system is designed for time-sensitive environments like vehicular networks, aerial drones, etc., where \textit{signers} are resource-limited (e.g., limited CPU and insufficient power reserves) devices, \textit{verifiers} are tasked with scalable, real-time, and efficient authentication of numerous requests, all while the system ensures time valid PQ security.


%%%%%%%%%%%%%% System model figure %%%%%%%%%%%%%%
% \begin{figure}[ht!]
% 	\vspace{-2mm}
% 	\centering
% 	\includegraphics[width=0.5\textwidth, scale=1]{Figures/system_model.pdf}
% 	\vspace{-3mm}
% 	\caption{High-level description of \bfhors~scheme}
% 	\label{fig:systemmodel}
% \end{figure}


\noindent \textbf{Threat and Security Model:} Our threat model assumes an adversary $\Attacker$ equipped with the following capabilities:

\begin{itemize}[leftmargin=8pt]
    \item[-] \textit{Passive attacks:} Aim to monitor and interpret the output of the signature generation interface.
    \item[-] \textit{Active attacks:} Aim to interpret, forge, and modify messages and signatures sent from the signers. We assume that $\Attacker$ is equipped with a quantum computer.
\end{itemize}

We follow the Existential Unforgeability under Chosen Message Attacks ($\eucma$) for the security model: % \cite{SecProofs}.

\vspace{-2mm}
%%% EUCMA Definition
\begin{definition} \label{def:onetimeeucma} The one-time $\eucma$ ($\oeucma$) experiment for one-time signature \sgn~is defined as follows:

\begin{itemize}[leftmargin=8pt]
    \item[-] $(\sk, \pk, I_{\sgn}) \,\as\, \sgnkg(1^\kappa)$
    \item[-] $(m^*, \sigma^*) \,\as\, \Attacker^{\sgnsig_{sk}(.)}(\pk, I_{\sgn})$
    \item[-] $\Attacker$ wins the experiment with a maximum of one query allowed if $1 \as \sgnver(\pk, m^*, \sigma^*)$ and $m^*$ was not queried to the signing oracle $\sgnsig_{sk}(.)$.
\end{itemize}

\vspace{1mm}
\hspace{-7mm} $Succ^{\oeucma}_{\sgn}(\Attacker) = Pr[Expt^{\oeucma}(\Attacker) = 1]$
\hspace{-4mm} $InSec^{\oeucma}_{\sgn}(T) = \underset{\Attacker}{max}\{Succ^{\oeucma}_{\sgn}(\Attacker)\}$ $<$ $negl(T)$
\end{definition}



==> back.tex <==
mu time = 890 micro



sigtime_32 = 16*0.057900000000 + 890 
sigtime_64 = 32*0.099600000000 + 890
sigtime_128 = 64*0.172300000000 + 890

TIME SHA2 on 256 byte message||CTR: 0.205525000000
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

% HORSIC: mu32:2.48  mu64: 4 mu128:7.5

% TIME SHA2 on 256 byte message||CTR: 0.205525000000

% sigtime_32 +=  3*0.205525000000 + 0.205525000000
% sigtime_64 +=
% sigtime_128 +=




% \item HORST: KAPPA:32 -> t=64, k = 16, l =32, |f|=128 Blake2s-128, k+logt= 22, 2t-1 = 127, k(logt+1)=112 
% \item HORST: KAPPA:64 -> t=128, k = 32, l =64, |f|=160 Blake2s-160, k+logt=39, 2t-1 = 255, k(logt+1)=256
% \item HORST: KAPPA:128 -> t=256, k = 64, l =128,|f|=256  Blake2b-256, k+logt=72, 2t-1 = 511, k(logt+1)=576

%%%%%%%%%%%%%%%%%%%%% Chain syncronized -> Same as HORS
% d=1
% \item HORSE: KAPPA:32 ->  t=64, k = 16, l =32, |f|=128  Blake2s-128, k+logt = 22
% \item HORSE: KAPPA:64 ->  t=128, k = 32, l =64, |f|=160 Blake2s-160, k+logt = 39
% \item HORSE: KAPPA:128 -> t=256, k = 64, l =128, |f|=256  Blake2b-256, k+logt = 72


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \item HORSIC: KAPPA:32 -> t=64, k=11, z=12, w=z-(k-1) = 2  l =32, |f|=128  Blake2s-128, wt=128, mu=1.4 , log2mu=0.49, kw=22 , 
% \item HORSIC: KAPPA:64 -> t=128, k=19, z=20, w=z-(k-1) = 2, l =64, |f|=160 Blake2s-160, wt=256, mu=1.12 , log2mu=0.17, kw=38, 
% \item HORSIC: KAPPA:128 -> t=256, k=32, z=33, w=z-(k-1) = 2, l =128, |f|=256  Blake2b-256, wt=512 , mu=1.16, log2mu=0.69, kw=64


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \item HORSIC+: KAPPA:32 (48) -> n=256 , t=64, k = 11, z=12 , w=z-(k-1) = 2  l=32, |f|=128  Blake2s-128, wt=128, kw=22
% \item HORSIC+: KAPPA:64 (77) -> n=256, t=128, k = 18, z=19 , w=z-(k-1) = 2, l =64, |f|=160 Blake2s-160, wt256, kw=36
% \item HORSIC+: KAPPA:128 (143) -> n=256, t=256, k = 32, z=33 , w=z-(k-1) = 2, l =128, |f|=256  Blake2b-256, wt=512 kw=64

% \item SHA2 on 32bit: 0.203373000000
% \item SHA2 on 64bit: 0.202094000000
% \item SHA2 on 128bit: 0.199285000000

% HORS finding CTR time





\section{Introduction}

The emergence of Internet of Things (IoT) devices, encompassing medical implants, personal gadgets like smartwatches, and military equipment such as aerial drones, significantly contributes to developing intelligent infrastructure in modern ubiquitous systems. These systems rely on Next Generation (NextG) networks integrating mobile devices and extensive data acquisition and control capabilities, underscoring the necessity for highly efficient protocols to ensure data integrity in a real-time manner (time-critical authentication). For instance, in vehicular networks (as an extension of the Internet of Vehicles (IoV)), immediate verification of messages among vehicles and infrastructure is essential for prompt responses to events such as sudden braking, crucial for accident prevention \cite{HacTimeValidVehic}. Other applications like transmitting command and control messages within time-sensitive Micro-smart grids \cite{Yavuz:SmartGrid:2015:Velin:MicroGrid}, power grids \cite{camara2016multicast}, and battery-powered aerial drones \cite{ozmen2018dronecrypt}, etc, emphasize the importance of real-time authentication. Therefore, there exists a demand for a real-time authentication mechanism that fulfills the following requirements and properties:





% Therefore, while ensuring the authenticity and integrity of exchanged messages is vital to prevent devastating attacks such as message tampering, false message injection, impersonation, and man-in-the-middle attacks, efficient authentication system is required. 

% Therefore, ensuring the authentication and integrity of such NextG networks while maintaining efficient operation is paramount.
% must adhere to real-time safety criteria. 
% Time-critical (delay-aware) operations are essential in various real-life applications. 

% For instance, efficient authentication mechanims are vital for or transmitting command and control messages within time-sensitive Micro-smart grids \cite{Yavuz:SmartGrid:2015:Velin:MicroGrid,saxena2017efficient}, the CAN bus standard in automotive communication systems \cite{Yavuz:ESCAR:SecuritySafety}, edge-based applications \cite{nakkar2020lightweight}, power grids \cite{TVHORS,TVOTS,camara2016multicast}, and battery-powered aerial drones \cite{ozmen2018dronecrypt,won2015secure}. 
% \cite{HacTimeValidVehic,li2013fadec,its2013ieee}
% \cite{TESLAPerrig,muTESLANing,tesfay2017experimental}

% Time-critical (delay-aware) operations are essential for various real-life applications. For example, in vehicular networks (as an extension of the Internet of Vehicles (IoV)), rapid (immediate) verification of messages across vehicles and infrastructure is vital for prompt responses to events such as sudden braking \cite{HacTimeValidVehic,li2013fadec,its2013ieee}. In IoV, ensuring the authenticity and integrity of the messages exchanged across the entities is critical to prevent potentially devastating attacks such as message tampering, false message injection, impersonation, and man-in-the-attack. To mitigate these vulnerabilities, broadcast authentication methods are used to prevent impersonation attacks and verify message integrity \cite{TESLAPerrig,muTESLANing,tesfay2017experimental}. Among those, digital signatures are one of the essential tools to ensure a scalable broadcast authentication~\cite{Vehicular:ECDSA:Manvi:2009}. In addition to vehicular networks, efficient authentication mechanisms are essential for transmitting command and control messages within time-sensitive Micro-smart grids \cite{Yavuz:SmartGrid:2015:Velin:MicroGrid,saxena2017efficient}, the CAN bus standard in automotive communication systems \cite{Yavuz:ESCAR:SecuritySafety}, edge-based applications \cite{nakkar2020lightweight}, power grids \cite{TVHORS,TVOTS,camara2016multicast}, and battery-powered aerial drones \cite{ozmen2018dronecrypt,won2015secure}. Therefore, there is a need for a real-time authentication mechanism that can satisfy the following requirements and properties:

% To mitigate these vulnerabilities, digital signatures are one of the essential tools to ensure scalable broadcast authentication \cite{Vehicular:ECDSA:Manvi:2009}. Additionally, efficient authentication mechanisms are vital f
% broadcast authentication methods are used to prevent impersonation attacks and verify message integrity. 
% Among these methods, digital signatures are one of the essential tools to ensure scalable broadcast authentication \cite{Vehicular:ECDSA:Manvi:2009}. 
Consequently, a real-time authentication mechanism should satisfy specific requirements and properties:

\underline{{\em Suitability to Real-Time (Time Valid) Characteristics:}} 
% The time-critical nature of applications like vehicular networks \cite{HacTimeValidVehic}, aerial drones \cite{ozmen2018dronecrypt}, etc, necessitates immediate transmission of messages once an endpoint creates them. Subsequently, these messages must be efficiently verified by the receiving endpoint. This also leads to some special authentication characteristics, in which the transmitted messages must remain secure only for a short period. For example, when a command is sent over a smart-grid system, the message and its digital signature must be transmitted and verified within a few milliseconds (at most). Beyond this time duration, the adversary loses its advantage of exploiting the delay-aware aspects of the application (e.g., triggering a malicious action on the smart grid, influencing system behavior timely). Hence, time valid applications, such as command authentications in smart grid and vehicular systems, may prioritize high-speed over long-term security as long as the security mechanism remains secure in a designated time interval. The prioritization of speedy authentication over long-term security is to ensure safety by minimizing the impact of the authentication overhead on the system's reliability. Note that, as discussed in the following sections, after real-time (delay-aware) verification under time valid constraints, one can later also ensure the long-term security of the messages for historical validation purposes (e.g., to enable audits). 
% Time-critical applications such as vehicular networks \cite{HacTimeValidVehic} and aerial drones \cite{ozmen2018dronecrypt} require immediate message transmission upon creation by an endpoint, followed by efficient verification by the receiving endpoint. This requirement results also in unique authentication characteristic, where transmitted messages must remain secure only for a short duration. For instance, in a smart-grid system, command messages and their digital signatures must be transmitted and verified within milliseconds. Beyond this time frame, potential adversaries lose the opportunity to exploit delay-aware aspects of the application (e.g., triggering a malicious action on the smart grid, influencing system behavior timely). Therefore, to minimize the impact of authentication overhead on system reliability, time-valid applications may prioritize speed over long-term security as long as the security mechanism remains effective within a designated time interval. Hence, {\em one of the main focuses of our work is to enable fast and secure digital signature functionality that must remain valid only for a limited amount of time, yet can also counter highly resourceful adversaries under such conditions}. It is important to note that, after real-time verification under time-valid constraints, measures can be implemented for long-term message security, enabling historical validation such as audits. % This prioritization aims to enhance safety by  


% Hence deleted
Time-critical applications such as vehicular networks \cite{HacTimeValidVehic} and aerial drones \cite{ozmen2018dronecrypt} necessitate immediate message transmission upon creation by an endpoint, followed by efficient verification by the receiving endpoint. This requirement leads to unique authentication characteristic, where transmitted messages must remain secure for only a short duration. For instance, in a smart-grid system, command messages and their digital signatures must be transmitted and verified within milliseconds. Beyond this time frame, potential adversaries lose the opportunity to exploit delay-aware aspects of the application, such as triggering a malicious action on the smart grid or influencing system behavior. Therefore, to minimize the impact of authentication overhead, time-valid applications may prioritize speed over long-term security, as long as the security mechanism remains effective within a designated time interval. It is important to note that, after real-time verification under time-valid constraints, measures can be implemented for long-term message security, enabling historical validation such as audits.




% Integrated Scalable as a word
\underline{{\em Computation and Communication Efficiency:}} High-speed authentication benefits real-time applications by minimizing end-to-end delay, which is mainly the compromise of the time required by generating, transmitting, and verifying signatures. Hence, a scalable computationally efficient digital signature with short tag sizes is ideal for delay-aware applications that follow the time valid concept. In addition to minimizing delay, some IoT end devices typically possess limited resources, including less powerful CPUs and inadequate power reserves for intensive computations. Therefore, an efficient authentication mechanism for these infrastructures is critical.

% % \underline{{\em Scalability:}} 
% Given that numerous envisioned time valid applications encompass many devices and systems, it becomes important for devices within these networks to respond to or initiate a considerable volume of authentications quickly within a restricted time frame. Scalable broadcast authentication is usually achieved via digital signatures.

% \underline{{\em Advanced Security Properties:}} Certain digital signatures offer specialized and enhanced security features, albeit at a higher cost, due to the additional operations compared to their traditional counterparts.

\ul{\em Post-quantum Security under Time Valid Settings:} 
% The emergence of quantum computers poses a significant threat to traditional cryptosystems due to Shor's algorithm \cite{Shor-algo,darzi2023envisioning}, capable of efficiently solving the hard problems underlying these systems, such as the (elliptic curve) discrete logarithm problem and integer factorization. In response, NIST initiated efforts to standardize post-quantum secure digital signatures \cite{nistCallProposals}, ending in the selection of three schemes: CRYSTALS-Dilithium \cite{ducas2018crystals}, FALCON \cite{fouque2019fast}, and SPHINCS+ \cite{aumasson2019sphincs} \cite{nistSelectedAlgorithms}. Despite this progress, NIST announced a continuation of the standardization process with a fourth-round \cite{nistStandardizationAdditional}. However, while efficient quantum-safe signature schemes like Dilithium \cite{Dilithium} offer robust security, their computational demands make them impractical for low-end IoT devices. Hence, IoT systems should prioritize post-quantum security solutions tailored for time valid settings, ensuring security for short durations while maintaining computational and communication efficiency.
The rise of quantum computers poses a significant threat to traditional digital signatures founded on conventional hard problems like prime factorization and discrete logarithm problems are vulnerable to quantum attacks such as Shor's algorithm \cite{Shor-algo}. To counter this, NIST embarked on standardizing post-quantum (PQ) secure digital signatures \cite{nistCallProposals,darzi2023envisioning}, ultimately selecting signature schemes like CRYSTALS-Dilithium \cite{ducas2018crystals}, FALCON \cite{fouque2019fast}, and SPHINCS+ \cite{aumasson2019sphincs}. Despite these advancements, NIST has announced a continuation of the standardization process with a fourth round \cite{nistStandardizationAdditional} to encourage diversity in signature standardization. 

% to conventional cryptosystems, thanks to algorithms like Shor's \cite{Shor-algo,darzi2023envisioning}, capable of swiftly solving the complex problems these systems rely on, such as the discrete logarithm problem and integer factorization. 
% \item {\em Forward-security}: Compromise-resiliency is a strong security feature that permits a cryptographic primitive to retain some security even after the keying material is compromised. Specifically, a forward-secure digital signature guarantees that the signatures generated before the key compromise happens remain unforgeable \cite{ForwardSecure_MMM_02}. This property can be highly beneficial for IoT applications, wherein the IoT end devices are vulnerable to key compromises~\cite{Yavuz:2012:TISSEC:FIBAF}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Related Work and Limitations of the State-of-the-Art}
% Two primary cryptographic techniques, namely HMAC \cite{ModernCryptoBellareRogaway} and symmetric ciphers \cite{StinsonCrypto}, are widely employed in wireless networks and IoT systems due to their computational efficiency. However, while suitable for smaller-scale setups, these methods encounter scalability challenges in large-distributed time valid systems and lack public verifiability. These restrict their applicability in scenarios necessitating non-repudiation, such as Visa, which manages numerous daily transactions requiring multiple authentications across diverse entities \cite{creditcardsDebitCard,wallethubCreditCard}. In contrast, digital signatures like ECDSA \cite{ECDSA}, EdDSA \cite{EdDSA}, RSA \cite{RSA}, and BLS \cite{BLS:2001} depend on Public Key Infrastructure (PKI) for verifying signatures, providing public verifiability, scalability for large systems, and ensuring non-repudiation. Hence, they are essential authentication mechanisms for security-critical applications such as medical devices, payment systems, and secure auditing in embedded devices. However, despite their capability to meet scalability and time valid needs, they face limitations: 

% Two primary cryptographic techniques, HMAC \cite{ModernCryptoBellareRogaway} and symmetric ciphers \cite{StinsonCrypto}, are commonly used in WSNs and IoT systems due to their computational efficiency. However, while suitable for smaller-scale setups, these methods face scalability challenges in large-distributed time-valid systems and lack public verifiability. These limitations restrict their applicability in scenarios necessitating non-repudiation, such as Visa transactions \cite{creditcardsDebitCard}. In contrast, digital signatures like ECDSA \cite{ECDSA}, EdDSA \cite{EdDSA}, RSA \cite{RSA}, and BLS \cite{BLS:2001} rely on Public Key Infrastructure (PKI) for verifying signatures, providing public verifiability, scalability for large systems, and ensuring non-repudiation. 
Despite their capability to meet scalability and time-valid needs, they encounter limitations:

\ul{\em Expensive operations in Conventional Digital Signatures:} 
% Public Key Cryptography (PKC)-based digital signatures (e.g., ECDSA, RSA) require costly operations like exponentiations and elliptic curve scalar multiplications, significantly more expensive than symmetric cryptography approaches \cite{ModernCryptoBellareRogaway}. Despite their benefits, their computational and memory overhead poses a significant challenge for integration into IoT applications. For instance, RSA offers computational efficiency during verification but demands expensive operations during signing, alongside large key and signature sizes, making it unsuitable for medical implant deployments. Conversely, ECDSA, with smaller key and signature sizes, may be preferred for better efficiency than RSA. However, despite the availability of various curves with different computational efficiency and security implemented on IoT devices (e.g., 8-bit AVR microprocessors \cite{Ed25519AVR,Kummer8bit,FourQ8bit}), these schemes still involve costly signing operations.
Public Key Cryptography (PKC)-based digital signatures, such as ECDSA and RSA, require computationally expensive operations like exponentiations and elliptic curve scalar multiplications, which are considerably more costly than symmetric cryptography approaches \cite{ModernCryptoBellareRogaway}. Moreover, their computational and memory overhead poses a significant challenge for time valid applications. For example, RSA offers computational efficiency during verification but demands expensive operations during signing, along with large key and signature sizes, rendering it unsuitable for medical implant deployments. Conversely, ECDSA, with smaller key and signature sizes, may be preferred for better efficiency than RSA. However, despite the availability of various curves with different computational efficiency and security implemented on IoT devices (e.g., 8-bit AVR microprocessors \cite{Ed25519AVR,Kummer8bit,FourQ8bit}), these schemes still involve costly signing operations.



\ul{\em Need for PQ Security and Challenges of High-Cost:} 
% Quantum computers present a significant threat to various sectors, including finance, IoT, government, and defense, as conventional cryptosystems like ECDSA, RSA, and EdDSA will no longer be secure \cite{darzi2023envisioning}. Although NIST has standardized post-quantum secure digital signatures (e.g., Dilithium \cite{Dilithium:2018}), they are computationally expensive, requiring heavy operations such as Gaussian Sampling \cite{NTRU:BLISS:Ducas:Crypto:2013}, and their key/signature sizes might be prohibitive for resource-constrained devices \cite{Tachyon,courtois2001achieve}. Although they offer long-term security against quantum attackers, they might become suitable for resource-constrained devices if their sizes are reduced. There are also some recent lightweight PQC signature schemes (e.g., \cite{ANT:ACSAC:2021,HASES,HASESACMTOMM}). However, they rely on special assumptions such as the presence of non-colluding distributed verification servers and/or secure hardware. All these cost concerns and special assumptions made existing PQC solutions hard to adapt to delay-aware and time valid settings. 
Although NIST has standardized post-quantum secure digital signatures (e.g., Dilithium \cite{Dilithium:2018}), they are computationally expensive, requiring heavy operations such as Gaussian Sampling \cite{NTRU:BLISS:Ducas:Crypto:2013}, and their key/signature sizes might be prohibitive for resource-constrained devices \cite{Tachyon,courtois2001achieve}. Consequently, real-time IoT systems must prioritize PQ security solutions tailored for time-valid settings, ensuring security for short durations while maintaining computational and communication efficiency. While there exists lightweight PQC signature schemes (e.g., \cite{ANT:ACSAC:2021,HASES,HASESACMTOMM}),  however, they rely on special assumptions such as the presence of non-colluding distributed verification servers and/or secure hardware. All these cost concerns and special assumptions has made existing PQC solutions hard to adapt to delay-aware and time-valid settings.
% Although they offer long-term security against quantum attackers, they might become suitable for resource-constrained devices if their sizes are reduced. % However, while potent quantum-safe signature schemes like Dilithium \cite{Dilithium} ensure robust security, their computational demands render them impractical for low-end IoT devices. 

\ul{\em Lightweight Conventional Signatures and Lack of Post-quantum Security:}  There are several commendable efforts in creating lightweight digital signatures that improve their conventional-secure counterparts (e.g., ECDSA, SchnorrQ). These usually involve advanced pre-computation and/or storage techniques as shown in CEDA~\cite{Yavuz:CEDA:2018}, ARIS~\cite{Yavuz:ARIS:2019}, SEMECS~\cite{SEMECS}, ETA~\cite{Yavuz:2013:EET:2462096.2462108}, BAF~\cite{BAFYavuzNing09}, and \cite{10.1145/3576842.3582376}. 


{\em Our literature review reveals a significant gap in simultaneously achieving all the desirable properties for achieving efficient digital signatures in time valid IoT environments. Therefore, there is a pressing demand for an ideal digital signature that meets the above desirable properties without relying on assumptions that may not hold in diverse real-world scenarios, all while maintaining a lightweight design.}



\subsection{Our Contribution}
Hash-based signatures have attracted increased attention due to their advantage in balancing signature size, execution time, and memory overhead to fulfill specific application requirements. For instance, while some hash-based signatures such as HORS \cite{HORS}, offer efficient signature generation and verification, others like SPHINCS \cite{SPHINCS:Bernstein:2015} and XMSS \cite{XMSS:Buchmann:2011} provide high security but entail very large signature sizes and costly signing processes. Given this advantage, we created a lightweight post-quantum signature named Time Valid Probabilistic Data Structure HORS (\bfhors) tailored for time valid IoT applications which entails the following properties:

\ul{\em Faster signature verification:} Leveraging the computational efficiency of \ohbf~for insertion and existence check of elements enhances the signature verification process within \hors, especially for the time valid settings. Our strategic use of \ohbf~as the One-way Function (OWF), combined with only $k<t$ calls to \ohbf~in the signature verification, permitted \bfhors~to fully benefit from the efficiency of underlying non-cryptographic hash function and modular operations. %For example, the resulting verification algorithms offer improvement around 5$\times$ with lower parameters (e.g., 32-bit time valid suited), 5$\times$ efficiency for moderate security levels (e.g., 64), and 2$\times$ with high-security parameters.


\ul{\em Faster Key Generation with Equal Signing Performance:} The principles outlined in signature verification also benefit the key generation, with the only difference being in total $t$ \ohbf~call is made. This permits a faster key generation compared to \hors~in low to moderate security levels (e.g., 32-bits to 64-bits) and comparable performance for higher security levels (e.g., 96-bits and 128-bits). Finally, our scheme maintains the signature generation efficiency of \hors~at any security level. 

\ul{\em Time valid PQ security:} \bfhors achieves PQ security tailored for time valid applications such that in contrast to PQ secure signatures (e.g., Dilithium), the impact of authentication overhead is eliminated by prioritizing speed over long-term security, as long as the security mechanism remains effective within a designated time interval



% Despite their merits, these schemes are not post-quantum secure. Furthermore, ECC-based primitives, although the most compact, are also among the most vulnerable against quantum computers (even more so than RSA-based methods) \cite{bernsteinRSAPostPQC,QuantumCircuitDLP,FactorRSA,proos2003shor}. Therefore, when they are used in time valid settings (e.g., \cite{TinyECC}) with smaller security parameters (to attain efficiency), their security degrades significantly faster than that of time valid solutions that can be constructed from PQC primitives (e.g., hash-based~\cite{HORS}). Moreover, time valid PQC primitives perform faster than even standardized curves. For instance, timings for curve secp160k1 \cite{SEGCECCurves} (160-bit security) is 110.88$\mu s$ for key generation, 116.85 $\mu s$ for signature generation, and 116.14 $\mu s$ for signature verification. Corresponding timings for curve secp256k1 \cite{SEGCECCurves} (256-bit security) is 219.91 $\mu s$ for key generation, 235.81 $\mu s$ for signature generation, and 215.78 $\mu s$ for signature verification (See Section \ref{sec:scheme1} for hardware and software configuration used for performance evaluation). In contrast, based on our experiments detailed in section \ref{sec:scheme1}, the timing for key generation is 6.6 $\mu s$, signature generation is 0.2 $\mu s$ and signature verification is 2.62 $\mu s$ for 128-bit security. This illustrates at least 3$\times$ faster key generation, 580 $\times$ faster signature generation, and 27$\times$ times signature verifications. Hence, in the following, we will turn our attention to PQC solutions with the best potential to serve as a building block for time valid applications.\\

% \vspace{2mm}
% \noindent \textbf{Hash-based Signatures as the Building Block for Time Valid Primitives in Post-quantum Settings:}  Due to the limitations of existing solutions (PKC-based digital signatures) in meeting the requirements of time valid systems, there is a critical demand for constructions tailored to time-critical needs. 

% Another line in digital signature construction involves utilizing hash functions (hash-based signatures) \cite{HBSSurvey,HBSReview}, which are post-quantum secure. Hash-based signatures have attracted increased attention due to the conciseness and efficiency of their underlying hash functions. Their advantage lies in balancing signature size, execution time, and memory overhead to fulfill specific application requirements. For instance, while some hash-based signatures such as \cite{HORS,HORSIC,Winternitz:Sec:buchmann2011security} offer efficient signature generation and verification (with limited number of signing), others like \cite{SPHINCS:Bernstein:2015,SPHINCS_ARM,XMSS:Buchmann:2011} provide high security with longer usage but entail very large signature sizes and costly signing processes. We focus on the following types of hash-based digital signatures based on the number of times they can be utilized upon instantiating their key pairs:

% \begin{itemize}
% \item {\em One-time Signatures (OTS):} The first OTS was proposed by Lamport in 1979 \cite{Lamport79}, aiming to minimize calculation costs and storage requirements. Merkle enhanced Lamport's scheme by introducing an additional checksum value, recording the number of zero bits in each message before signing, and reducing signature and key pair sizes \cite{MerkleOTS}. Subsequently, Winternitz OTS (W-OTS) \cite{Winternitz:Sec:buchmann2011security} further refined the Lamport and Merkle schemes, achieving even shorter signature and key pair sizes. However, W-OTS required additional hash evaluations. A subsequent advancement, W-OTS+ \cite{hulsing2013optimal}, maintained a similar security level while producing even shorter signatures compared to previous schemes. These developments aimed to optimize signature sizes while balancing computational efficiency and security.

% \item {\em Few-time Signatures (FTS):} Hash-based FTSs enable multiple messages to be signed using the same key pair, although the security decreases with the number of signed messages. The first FTS was BiBa \cite{BiBa}, which prioritized fast verification and small signature size but at the expense of signature generation time and public key size. Later, HORS \cite{HORS} extended the Lamport OTS by using Bos-Chaum signatures and cover-free families. With the vulnerability of HORS against using weak messages \cite{HORSWeakMessageAttack}, PORS \cite{aumasson2018improving} and FORS \cite{SPHINCS+} addressed this vulnerability by employing a pseudorandom subset obtained using a pseudorandom number generator. Moreover, HORS has been fundamentally used in schemes like HORST \cite{SPHINCS:Bernstein:2015}, HORSIC \cite{HORSIC}, HORSIC+ \cite{lee2021horsic+}, \cite{InfHORS} etc., in recent years. The properties of HORS have led to its use in developing authentication systems (e.g., TV-HORS \cite{TVHORS}) for time-sensitive multicast data, where minimizing end-to-end delay, ensuring computational and communication efficiency, and packet loss resiliency is vital. 

% \item {\em Many-time Signatures (MTS):} A MTS uses one or more OTS/FTS schemes as its building block. Merkle Signature Scheme (MSS) \cite{MSS} is built upon WOTS and reduced key and signature sizes to a practical level and incorporated hash trees to allow for reusing a single public key for a specific number of times (many times). Some variants of MSS are XMSS \cite{XMSS}, which reduced key and signature sizes and incorporated a more secure version of the hash tree. XMSS uses a compact variant of WOTS as its building block. More advanced MSS schemes, like XMSS$^{MT}$ \cite{XMSSmt}, SPHINCS \cite{SPHINCS}, SPHINCS+ \cite{SPHINCS+}, allow reusing a single public key for a polynomially unbounded number of times.  

% \end{itemize}


% {\em The analysis of state-of-the-art signatures shows that hash-based signatures are the best alternative to build time valid digital signatures for delay-aware applications. Despite their merits, full-fledge signature primitives such as SPHINCS+ and XMSS (with their variants) are extremely costly for delay-aware applications. There are limited alternatives for time valid hash-based signatures (e.g., TV-HORS \cite{TVHORS}) offering security trade-offs only in a limited range, requiring relatively tighter time synchronization as well as still incurring non-negligible running times. Hence, there is a critical need to develop post-quantum secure time valid signatures that can offer high performance on a broad range of security parameters towards meeting the needs of delay-aware applications.}











































%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% T1 %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t] 
    \centering
    \scriptsize
 
    \caption{Performance comparison of \bfhors~and \hors~($f()$: SHA2 family)} 
    \label{tab:perfsha2}
    
    \vspace{-2mm}
	
    \begin{tabular}{| c | c | c | c | c | c| c | c | c | c | c |}
        \hline

        \textbf{Scheme} & \textbf{(t, k, l, p)} &  \textbf{H(.)}   \textbf{f(.) or h(.)} & \textbf{PK (KB)}  &  \textbf{Key Gen (\bm{$\mu$}s)} & \textbf{Sig Ver (\bm{$\mu$}s)} & \bm{$\kappa$} \\ \hline \hline
        
        \specialcell[]{\hors \\ \bfhors} & (64, 16, 32, 8) & \specialcell[]{  SHA2-256    SHA2-256 \\    SHA2-256    xxHash3-64} & \specialcell[]{2 \\ {0.971}} & 
        \specialcell[]{12.08 \\ {1.99}}  & \specialcell[]{3.11 \\ {0.66}} & 32 \\ \hline 
                        
        \specialcell[]{\hors \\ \bfhors} & (64, 32, 32, 8) & \specialcell[]{   SHA2-256    SHA2-256 \\    SHA2-256    xxHash3-64} & \specialcell[]{2 \\ {0.971}} & \specialcell[]{13.14 \\ {1.96}} &  \specialcell[]{6.32 \\ {1.28}} & 32 \\ \hline 
                        
        \specialcell[]{\hors \\ \bfhors} & (128, 16, 48, 17) & \specialcell[]{   SHA2-256    SHA2-256 \\    SHA2-256    xxHash3-128} & \specialcell[]{4 \\ {1.87}} & \specialcell[]{24.99 \\ {10.45}} &  \specialcell[]{3.15 \\ {0.709}} & 48 \\ \hline 
                        
        \specialcell[]{\hors \\ \bfhors} & (256, 16, 64, 28) & \specialcell[]{   SHA2-256    SHA2-256 \\    SHA2-256    xxHash3-128} & \specialcell[]{8 \\ {3.93}} & \specialcell[]{48.08 \\ {30.84}} &  \specialcell[]{3.13 \\ {0.647}} & 64 \\ \hline 
                        
        \specialcell[]{\hors \\ \bfhors} & (128, 32, 64, 28) & \specialcell[]{   SHA2-256    SHA2-256 \\    SHA2-256    xxHash3-128} & \specialcell[]{4 \\ {1.95}} & \specialcell[]{24.03 \\ {16.23}} &  \specialcell[]{6.19 \\ {1.3}} & 64 \\ \hline 

        \hline\hline

        \specialcell[]{\hors \\ \bfhors} & (512, 16, 72, 36) & \specialcell[]{   SHA2-256    SHA2-256 \\    SHA2-256   CityHash256} & \specialcell[]{16 \\ {7.9}} & \specialcell[]{98.37 \\ {87.96}} &  \specialcell[]{3.17 \\ {1.12}} & 72 \\ \hline 
            
        \specialcell[]{\hors \\ \bfhors} & (256, 32, 96, 38) & \specialcell[]{   SHA2-256    SHA2-256 \\    SHA2-256   CityHash256} & \specialcell[]{8 \\ {5.44}} & \specialcell[]{46.89 \\ {45.81}} &  \specialcell[]{6.01 \\ {2.19}} & 96 \\ \hline 

        \specialcell[]{\hors \\ \bfhors} & (512, 32, 128, 28) & \specialcell[]{   SHA2-512    Blake2b-256 \\    SHA2-512    CityHash256} & \specialcell[]{16 \\ {40.73}} & \specialcell[]{71.52 \\ {72.48}} &  \specialcell[]{4.65 \\ {2.29}} & 128 \\ \hline 
                        
        \specialcell[]{\hors \\ \bfhors} & (256, 64, 256, 30) & \specialcell[]{   SHA2-512    Blake2b-256 \\    SHA2-512   CityHash256} & \specialcell[]{8 \\ {17.58}} & \specialcell[]{36.22 \\ {37.66}} &  \specialcell[]{9.12 \\ {4.37}} & 128 \\ \hline 
	
    \end{tabular}
	
	
\begin{tablenotes}[flushleft] \scriptsize{
\item  Message size: 256 Bytes. The $n$ is the PK size.
The private key size for both the \hors~and \bfhors~is computed as $t\cdot l$. However, in practice, private keys are generated from a seed of constant size. Thus, the private key's size is considered constant. The PK column for \bfhors~shows the size of the \ohbf. The signature size for both \hors~and \bfhors~is computed as $k \cdot l$ plus the size of the $Ctr$ variable. The signature generation time for both \hors~and \bfhors~is the same since all functionalities are identical. Despite adding resistance against weak message attacks in \bfhors~, we can also incorporate this enhancement into \hors.
}

	\end{tablenotes}
\end{table*}	




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% T2 %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
    \centering
    \scriptsize
 
    \caption{Performance comparison of \bfhors~and \hors~($f()$: Blake2 family)}
    \label{tab:perfblake}
    \vspace{-2mm}
	
    \begin{tabular}{| c | c | c | c | c | c| c | c | c | c | c |}
    \hline
        
        \textbf{Scheme} & \textbf{(t, k, l, p)} &   \textbf{H(.)}    \textbf{f(.) or h(.)}    & \textbf{PK (KB)}  &  \textbf{Key Gen (\bm{$\mu$}s)} & \textbf{Sig Ver (\bm{$\mu$}s)} & \bm{$\kappa$} \\ \hline \hline

        \specialcell[]{\hors \\ \bfhors} & (64, 16, 32, 8) & \specialcell[]{   SHA2-256    Blake2s-128 \\    SHA2-256    xxHash3-64} & \specialcell[]{1 \\ {0.971}} & 
       \specialcell[]{8.51 \\ {1.99}}  & \specialcell[]{1.85 \\ {0.66}} & 32 \\ \hline 
                        
        \specialcell[]{\hors \\ \bfhors} & (64, 32, 32, 8) & \specialcell[]{   SHA2-256    Blake2s-128 \\   SHA2-256    xxHash3-64} & \specialcell[]{1 \\ {0.971}} & \specialcell[]{7.92 \\ {1.96}} &  \specialcell[]{3.69 \\ {1.28}} & 32 \\ \hline 
                        
        
        \specialcell[]{\hors \\ \bfhors} & (128, 16, 48, 17) & \specialcell[]{   SHA2-256    Blake2s-128 \\   SHA2-256    xxHash3-128} & \specialcell[]{2 \\ {1.87}} & \specialcell[]{15.17 \\ {10.45}} &  \specialcell[]{1.81 \\ {0.709}} & 48 \\ \hline 
                        

        \specialcell[]{\hors \\ \bfhors} & (256, 16, 64, 28) & \specialcell[]{   SHA2-256    Blake2s-128 \\   SHA2-256    xxHash3-128} & \specialcell[]{4 \\ {3.93}} & \specialcell[]{29.55 \\ {30.84}} &  \specialcell[]{1.85 \\ {0.647}} & 64 \\ \hline 
                        
        
        \specialcell[]{\hors \\ \bfhors} & (128, 32, 64, 28) & \specialcell[]{   SHA2-256    Blake2s-128 \\   SHA2-256    xxHash3-128} & \specialcell[]{2 \\ {1.95}} & \specialcell[]{15.28 \\ {16.23}} &  \specialcell[]{3.65 \\ {1.3}} & 64 \\ \hline 

        \hline\hline

        \specialcell[]{\hors \\ \bfhors} & (512, 16, 72, 30) & \specialcell[]{   SHA2-256    Blake2s-160 \\   SHA2-256    CityHash256} & \specialcell[]{10 \\ {6.28}} & \specialcell[]{58.02 \\ {76.5}} &  \specialcell[]{1.91 \\ {1.14}} & 72 \\ \hline 
            

        \specialcell[]{\hors \\ \bfhors} & (256, 32, 96, 32) & \specialcell[]{   SHA2-256    Blake2b-256 \\   SHA2-256    CityHash256} & \specialcell[]{8 \\ {6.34}} & \specialcell[]{29.02 \\ {40.09}} &  \specialcell[]{3.68 \\ {2.22}} & 96 \\ \hline 
                        

        \specialcell[]{\hors \\ \bfhors} & (512, 32, 128, 28) & \specialcell[]{   SHA2-512    Blake2b-256 \\    SHA2-512    CityHash256} & \specialcell[]{16 \\ {40.73}} & \specialcell[]{71.52 \\ {72.48}} &  \specialcell[]{4.65 \\ {2.29}} & 128 \\ \hline 
                        

        \specialcell[]{\hors \\ \bfhors} & (256, 64, 256, 30) & \specialcell[]{   SHA2-512    Blake2b-256 \\    SHA2-512    CityHash256} & \specialcell[]{8 \\ {17.58}} & \specialcell[]{36.22 \\ {37.66}} &  \specialcell[]{9.12 \\ {4.37}} & 128 \\ \hline                       
    \end{tabular}
	
	
\begin{tablenotes}[flushleft] \scriptsize{
\item See the footnotes of the Table \ref{tab:perfsha2} for more details.
}

	\end{tablenotes}
\end{table*}	



==> notes.tex <==
% https://dl.acm.org/doi/pdf/10.1145/2462096.2462108?casa_token=yNsynuOjLIIAAAAA:RNtFYL4QiJTzwi54ctK-FuQ30TUyK5t-6i1-WLCh2AGjoQRSRW3l7STGgXTnLWlOTqbkoi-e6RvzaQ
% https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=6882222&casa_token=Lz_tIteoMnEAAAAA:IBr3k2nq0WtZMIaoVb5kgvIK3p_BTcwTXwRAGHEWEjxgALCdyf1HNEKS_cilxkJSEJu6U-vnWA

update Git
password protect


sha2
ebiba
HORS++
nistcall
saleh
shnorq website

